Neural Polar Decoders for Deletion Channels

This paper introduces a neural polar decoder (NPD) for deletion channels with a constant deletion rate. Existing polar decoders for deletion channels exhibit high computational complexity of $O(N^4)$, where $N$ is the block length. This limits the application of polar codes for deletion channels to short-to-moderate block lengths. In this work, we demonstrate that employing NPDs for deletion channels can reduce the computational complexity. First, we extend the architecture of the NPD to support deletion channels. Specifically, the NPD architecture consists of four neural networks (NNs), each replicating fundamental successive cancellation (SC) decoder operations. To support deletion channels, we change the architecture of only one. The computational complexity of the NPD is $O(AN\log N)$, where the parameter $A$ represents a computational budget determined by the user and is independent of the channel. We evaluate the new extended NPD for deletion channels with deletion rates $\delta\in\{0.01, 0.1\}$ and we verify the NPD with the ground truth given by the trellis decoder by Tal et al. We further show that due to the reduced complexity of the NPD, we are able to incorporate list decoding and further improve performance. We believe that the extended NPD presented here could have applications in future technologies like DNA storage.

==> figures/diagrams/communication-setting.tex <==
\begin{tikzpicture}[node distance=3.8cm and 2.5cm, auto, >=Latex]
    \node[minimum width=0.5cm, minimum height=1cm] (m) {$B^K$};
    \node[draw, rectangle, right=1.cm of m, minimum width=1.5cm, minimum height=1cm] (enc) {Encoder};
    \node[draw, rectangle, right=1.5cm of enc, minimum width=1.5cm, minimum height=1cm] (ch) {Channel};
    % \node[draw, rectangle, below=0.5cm of ch, minimum width=0.5cm, minimum height=0.5cm] (del) {$\Delta$};
    \node[draw, rectangle, right=1.5cm of ch, minimum width=1.5cm, minimum height=1cm] (dec) {Decoder};
    \node[right=0.5cm of dec, minimum width=0.5cm, minimum height=1cm] (mhat) {$\hat{B}^K$};
  
    % Arrows
    \draw[->] (m.east) --  (enc.west);
    \draw[->] (enc.east) -- node[above] {$X^N$} (ch.west);
    \draw[->] (ch.east) -- node[above](y) {$Y^D$} (dec.west);
    % \draw[->] (y.south) |- (del.east);
    % \draw[->, dashed] (del.west) -| (enc.south);
    \draw[->] (ch.east) -- node[above] {} (dec.west);
    \draw[->] (dec.east) --  (mhat.west);
    % \draw[->, thick] (3,1) .. controls (2.5,0.5) and (1,-0.5) .. (0.2,-1);

    % \draw[->] (dec.east) to[bend right=30] node[below] {Feedback} (enc.south);
  \end{tikzpicture}

==> figures/diagrams/nsc-training.tex <==
\tikzstyle{gn} = [rectangle,
                    node distance=1.5cm,
                    % rounded corners,
                    minimum width=1.5cm, 
                    minimum height=1.25cm,
                    minimum size=1.25cm,
                    % text width=0.25cm, 
                    text centered, 
                    draw=black,thin,
                    scale=1.0]
\tikzstyle{io} =    [node distance=0.5cm,
                    minimum height=0.25cm,
                    text centered,
                    scale=\scale]

\tikzset{XOR/.style={draw,circle,append after command={
        [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
        (\tikzlastnode.north) edge (\tikzlastnode.south)
        (\tikzlastnode.east) edge (\tikzlastnode.west)}}}

\tikzset{
    pics/nnops/.style=
    {
        code=
        {
        \node(#1)[gn] at (0,0){} ;
        \node (a) [io, at={($(#1.west)+(0.75em,1em)$)}, scale=1.5, thick] {$\scriptstyle \textcolor{boldblue}{F_\theta}$};
        \node (b) [io, at={($(#1.west)+(0.75em,-1em)$)}, scale=1.5, thick] {$\scriptstyle \textcolor{boldblue}{G_\theta}$};
        }
    }
} 

\def\scale{0.8}
\begin{tikzpicture}[
node distance = 3cm, 
auto,
]

\pic [] {nnops=Gn11};
\pic [right of=Gn11, xshift=1.cm] {nnops=Gn12};
\pic [below of=Gn11, xshift=0.cm, yshift=-0.05cm] {nnops=Gn21};
\pic [right of=Gn21, xshift=1.cm, yshift=0.0cm] {nnops=Gn22};


% %%%%%%%%%%%%% arrows %%%%%%%%%%%%%
\draw[->] ([yshift=0.28cm] Gn11.west) -- ++ (-3em, 0) node[anchor=east, pos=1, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]90:$\celoss{v_{2,1}}{e_{2,1}}$}] {${v_{2,1}},{e_{2,1}}$};
\draw[->] ([yshift=-0.25cm]Gn11.west) -- ++ (-3em, 0) node[anchor=east, pos=1, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]270:$\celoss{v_{2,2}}{e_{2,2}}$}] {${v_{2,2}},{e_{2,2}}$};
\draw[->] ([yshift=0.28cm] Gn21.west) -- ++ (-3em, 0) node[anchor=east, pos=1, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]90:$\celoss{v_{2,3}}{e_{2,3}}$}] {${v_{2,3}},{e_{2,3}}$};
\draw[->] ([yshift=-0.25cm]Gn21.west) -- ++ (-3em, 0) node[anchor=east, pos=1, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]270:$\celoss{v_{2,4}}{e_{2,4}}$}] {${v_{2,4}},{e_{2,4}}$};


\draw[<-] ([yshift=0.28cm]Gn11.east)  -- node[anchor=south, pos=0.75, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]90:$\celoss{v_{1,1}}{e_{1,1}}$}] {${v_{1,1}},{e_{1,1}}$} ([yshift=0.28cm]Gn12.west);
\draw[<-] ([yshift=0.28cm]Gn21.east)  --++ (0.5,0.0) --++ (0.75,2.515cm) -- node[anchor=south, xshift=-0.0cm, yshift=-0.0cm, scale=\scale, pos=0.6, pin={[pin edge={black, dashed, ->}, scale=\scale]270:$\celoss{v_{1,2}}{e_{1,2}}$}] {${v_{1,2}},{e_{1,2}}$} ([yshift=-0.25cm]Gn12.west);
\draw[<-] ([yshift=-0.25cm]Gn11.east)  --++ (0.5,0.0) --++ (0.75,-2.515cm) -- node[anchor=north, xshift=-0cm, yshift=0.0cm, scale=\scale, pos=0.55, pin={[pin edge={black, dashed, ->}, scale=\scale]90:$\celoss{v_{1,3}}{e_{1,3}}$}] {${v_{1,3}},{e_{1,3}}$} ([yshift=0.28cm]Gn22.west);
\draw[<-] ([yshift=-0.25cm]Gn21.east)  -- node[anchor=north, xshift=0.0cm, yshift=0.00cm, scale=\scale, pos=0.75, pin={[pin edge={black, dashed, ->}, scale=\scale]270:$\celoss{v_{1,4}}{e_{1,4}}$}] {${v_{1,4}},{e_{1,4}}$} ([yshift=-0.25cm]Gn22.west);

\draw[<-] ([yshift=0.28cm] Gn12.east)  -- ++ (3em, 0) node[right, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]90:$\celoss{v_{0,1}}{e_{0,1}}$}] (v1) {${v_{0,1}},{e_{0,1}}$};
\draw[<-] (v1.east)  -- ++ (1.5em, 0) node[above, scale=\scale] {$\textcolor{boldblue}{E_\theta}$} -- ++ (1.5em, 0) node[right, scale=\scale] {$y_1$};
\draw[<-] ([yshift=-0.25cm]Gn12.east)  -- ++ (3em, 0) node[right, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]270:$\celoss{v_{0,2}}{e_{0,2}}$}]  (v2) {${v_{0,2}},{e_{0,2}}$};
\draw[<-] (v2.east)  -- ++ (1.5em, 0) node[above, scale=\scale] {$\textcolor{boldblue}{E_\theta}$} -- ++ (1.5em, 0) node[right, scale=\scale] {$y_2$};
\draw[<-] ([yshift=0.28cm] Gn22.east)  -- ++ (3em, 0) node[right, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]90:$\celoss{v_{0,3}}{e_{0,3}}$}] (v3) {${v_{0,3}},{e_{0,3}}$};
\draw[<-] (v3.east)  -- ++ (1.5em, 0) node[above, scale=\scale] {$\textcolor{boldblue}{E_\theta}$} -- ++ (1.5em, 0) node[right, scale=\scale] {$y_3$};
\draw[<-] ([yshift=-0.25cm]Gn22.east)  -- ++ (3em, 0) node[right, scale=\scale, pin={[pin edge={black, dashed, ->}, scale=\scale]270:$\celoss{v_{0,4}}{e_{0,4}}$}] (v4) {${v_{0,4}},{e_{0,4}}$};
\draw[<-] (v4.east)  -- ++ (1.5em, 0) node[above, scale=\scale] {$\textcolor{boldblue}{E_\theta}$} -- ++ (1.5em, 0) node[right, scale=\scale] {$y_4$};
% \draw[-,dashed, semithick] ($(Gn11.south)-(3.5, 0.75)$) -- ($(Gn12.south)-(-3.5, 0.75)$);
\draw[-,dashed, semithick] ($(Gn11.east)+(0.88, 1.75)$) -- ($(Gn21.east)+(0.88, -1.75)$);
\draw[-,dashed, semithick] ($(Gn12.east)+(0.5, 1.75)$) -- ($(Gn22.east)+(0.5, -1.75)$);
% \draw[<-, dashed] (Ch1.north)  --++ (0.0, 0.5cm) node[anchor=south, scale=1.0] {$s_0$};
% \draw[->, dashed] (Ch1.south)  -- node[anchor=east, scale=1.0] {$s_2$} (Ch2.north);
% \draw[->, dashed] (Ch2.south)  --++ (0.0, -0.5cm) node[anchor=north, scale=1.0] {$s_4$};


\end{tikzpicture}

==> figures/diagrams/tikz-fig-npd.tex <==
\begin{tikzpicture}
        \foreach \x in {0.5, 2.5, 4.5, 6.5} {
            \fill[yellow!50] (\x, -3.5) rectangle ++(1, 7.5);
        }
        % Nodes for x values on the left
        \node[] at (1, 4.5) {$x_1$};
        \node[] at (3, 4.5) {$x_2$};
        \node[] at (5, 4.5) {$x_3$};
        \node[] at (7, 4.5) {$x_4$};
        % Nodes for y values on the left
        \node[blue] at (-1, 2) {$y_1 = 1$};
        \node[red] at (-1, 0) {$y_2 = 0$};
        \node[blue] at (-1, -2) {$y_3 = 1$};
    
        % Nodes representing dots
        \foreach \y in {3, 1, -1, -3} {
            \foreach \x in {0, 2, 4, 6, 8} {
                \node[circle, fill=black, inner sep=1pt] at (\x, \y) {};
            }
        }
        \draw (0, 3) circle (0.15cm);
        \draw (8, -3) circle (0.15cm);
        % Draw arrows with annotations
        % Red arrow from (0, 3) to (2, 1)
        \draw[->, red, thick] (0, 3) to[out=45, in=135]node[midway, above] {$\scriptstyle d / 2$}(2, 3);
        \draw[->, blue, thick] (0, 3) to[out=-45, in=-135]node[midway, above] {$\scriptstyle d / 2$}(2, 3);
        \draw[->, blue, thick] (0, 3) tonode[midway, above] {$\scriptstyle\bar{ d} / 2$}(2, 1);
        \draw[->, blue, thick] (2, 3) tonode[midway, above] {$\scriptstyle\bar{ d} / 2$}(4, 1);
        
        \draw[->, red, thick] (2, 1) to[out=45, in=135]node[midway, above] {$\scriptstyle d / 2$}(4, 1);
        \draw[->, blue, thick] (2, 1) to[out=-45, in=-135]node[midway, above] {$\scriptstyle d / 2$}(4, 1);
        \draw[->, red, thick] (2, 1) tonode[midway, above] {$\scriptstyle\bar{ d} / 2$}(4, -1);
        \draw[->, red, thick] (4, 1) tonode[midway, above] {$\scriptstyle\bar{ d} / 2$}(6, -1);
    
    
        \draw[->, red, thick] (4, -1) to[out=45, in=135]node[midway, above] {$\scriptstyle d / 2$}(6, -1);
        \draw[->, blue, thick] (4, -1) to[out=-45, in=-135]node[midway, above] {$\scriptstyle d / 2$}(6, -1);
        \draw[->, blue, thick] (4, -1) tonode[midway, above] {$\scriptstyle\bar{ d} / 2$}(6, -3);
        \draw[->, blue, thick] (6, -1) tonode[midway, above] {$\scriptstyle\bar{ d} / 2$}(8, -3);
        
        \draw[->, red, thick] (6, -3) to[out=45, in=135]node[midway, above] {$\scriptstyle d / 2$}(8, -3);
        \draw[->, blue, thick] (6, -3) to[out=-45, in=-135]node[midway, above] {$\scriptstyle d / 2$}(8, -3);
        % \draw[->, red, thick] (0, 3) to[out=30, in=150] (2, 1);
        % \node at (1, 3.5) {$ d / 2$};
        % % Blue arrow from (2, 1) to (0, -1)
        % \draw[->, blue, thick] (2, 1) to[out=210, in=330] (0, -1);
        % \node at (1, 0) {$ d / 2$};
    
        % % Additional arrows (red and blue for different connections)
        % \draw[->, red, thick] (2, 1) to[out=30, in=150] (4, 3);
        % \node at (3, 2.5) {$\overline{ d}/2$};
    
        % \draw[->, blue, thick] (4, 3) to[out=210, in=30] (2, -1);
        % \node at (3, 1) {$\overline{ d}/2$};
    
        % Add e labels below the columns
        \node at (1, -4) {$e_1$};
        \node at (3, -4) {$e_2$};
        \node at (5, -4) {$e_3$};
        \node at (7, -4) {$e_4$};
    
    \end{tikzpicture}

==> figures/diagrams/trellis-deletion.tex <==
\begin{tikzpicture}
    \foreach \x in {0.5, 2.5, 4.5, 6.5} {
        \fill[yellow!50] (\x, -3.5) rectangle ++(1, 7.5);
    }
    % Nodes for x values on the left
    \node[] at (1, 4.5) {$x_1$};
    \node[] at (3, 4.5) {$x_2$};
    \node[] at (5, 4.5) {$x_3$};
    \node[] at (7, 4.5) {$x_4$};
    % Nodes for y values on the left
    \node[blue] at (-1, 2) {$y_1 = 1$};
    \node[red] at (-1, 0) {$y_2 = 0$};
    \node[blue] at (-1, -2) {$y_3 = 1$};

    % Nodes representing dots
    \foreach \y in {3, 1, -1, -3} {
        \foreach \x in {0, 2, 4, 6, 8} {
            \node[circle, fill=black, inner sep=1pt] at (\x, \y) {};
        }
    }
    \draw (0, 3) circle (0.15cm);
    \draw (8, -3) circle (0.15cm);
    % Draw arrows with annotations
    % Red arrow from (0, 3) to (2, 1)
    \draw[->, red, thick] (0, 3) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(2, 3);
    \draw[->, blue, thick] (0, 3) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(2, 3);
    \draw[->, blue, thick] (0, 3) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(2, 1);
    \draw[->, blue, thick] (2, 3) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(4, 1);
    
    \draw[->, red, thick] (2, 1) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(4, 1);
    \draw[->, blue, thick] (2, 1) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(4, 1);
    \draw[->, red, thick] (2, 1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(4, -1);
    \draw[->, red, thick] (4, 1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(6, -1);


    \draw[->, red, thick] (4, -1) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(6, -1);
    \draw[->, blue, thick] (4, -1) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(6, -1);
    \draw[->, blue, thick] (4, -1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(6, -3);
    \draw[->, blue, thick] (6, -1) tonode[midway, above] {$\scriptstyle\bar{d} / 2$}(8, -3);
    
    \draw[->, red, thick] (6, -3) to[out=45, in=135]node[midway, above] {$\scriptstyled / 2$}(8, -3);
    \draw[->, blue, thick] (6, -3) to[out=-45, in=-135]node[midway, above] {$\scriptstyled / 2$}(8, -3);
    % \draw[->, red, thick] (0, 3) to[out=30, in=150] (2, 1);
    % \node at (1, 3.5) {$d / 2$};
    % % Blue arrow from (2, 1) to (0, -1)
    % \draw[->, blue, thick] (2, 1) to[out=210, in=330] (0, -1);
    % \node at (1, 0) {$d / 2$};

    % % Additional arrows (red and blue for different connections)
    % \draw[->, red, thick] (2, 1) to[out=30, in=150] (4, 3);
    % \node at (3, 2.5) {$\overline{d}/2$};

    % \draw[->, blue, thick] (4, 3) to[out=210, in=30] (2, -1);
    % \node at (3, 1) {$\overline{d}/2$};

    % Add e labels below the columns
    \node at (1, -4) {$e_1$};
    \node at (3, -4) {$e_2$};
    \node at (5, -4) {$e_3$};
    \node at (7, -4) {$e_4$};

\end{tikzpicture}
